Automated Machine Learning for Multi-Label Classification

Automated machine learning (AutoML) aims to select and configure machine learning algorithms and combine them into machine learning pipelines tailored to a dataset at hand. For supervised learning tasks, most notably binary and multinomial classification, aka single-label classification (SLC), such AutoML approaches have shown promising results. However, the task of multi-label classification (MLC), where data points are associated with a set of class labels instead of a single class label, has received much less attention so far. In the context of multi-label classification, the data-specific selection and configuration of multi-label classifiers are challenging even for experts in the field, as it is a high-dimensional optimization problem with multi-level hierarchical dependencies. While for SLC, the space of machine learning pipelines is already huge, the size of the MLC search space outnumbers the one of SLC by several orders. In the first part of this thesis, we devise a novel AutoML approach for single-label classification tasks optimizing pipelines of machine learning algorithms, consisting of two algorithms at most. This approach is then extended first to optimize pipelines of unlimited length and eventually configure the complex hierarchical structures of multi-label classification methods. Furthermore, we investigate how well AutoML approaches that form the state of the art for single-label classification tasks scale with the increased problem complexity of AutoML for multi-label classification. In the second part, we explore how methods for SLC and MLC could be configured more flexibly to achieve better generalization performance and how to increase the efficiency of execution-based AutoML systems.

==> content/acknowledgement.tex <==
% !TEX root = ../my-thesis.tex
%
\pdfbookmark[0]{Acknowledgement}{Acknowledgement}
\chapter*{Acknowledgement}
\label{sec:acknowledgement}
\vspace*{-10mm}



==> gfx/classifier-usages.tex <==

\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar, axis on top,
        title={Cumulative Progress of Works},
        height=8cm, width=15.5cm,
        bar width=0.4cm,
        ymajorgrids, tick align=inside,
        major grid style={draw=white},
        enlarge y limits={value=.1,upper},
        ymin=0, ymax=100,
        axis x line*=bottom,
        axis y line*=right,
        y axis line style={opacity=0},
        tickwidth=0pt,
        enlarge x limits=true,
        legend style={
            at={(0.5,-0.2)},
            anchor=north,
            legend columns=-1,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        ylabel={Percentage (\%)},
        symbolic x coords={
           Sep-11,Oct-11,Nov-11,Dec-11,
           Jan-12,Feb-12,
           Mar-12,
          Apr-12},
       xtick=data,
       nodes near coords={
        \pgfmathprintnumber[precision=0]{\pgfplotspointmeta}
       }
    ]
    \addplot [draw=none, fill=blue!30] coordinates {
      (Sep-11,75.4064)
      (Oct-11, 72.7961) 
      (Nov-11,94.4597)
      (Dec-11,66.6786) 
      (Jan-12,67.5600) 
      (Feb-12,88.2339)
      (Mar-12,78.6138) 
      (Apr-12,58.9129) };
   \addplot [draw=none,fill=red!30] coordinates {
      (Sep-11,75.4064)
      (Oct-11, 89.7961) 
      (Nov-11,94.4597)
      (Dec-11,76.6786) 
      (Jan-12,77.5600) 
      (Feb-12,78.2339)
      (Mar-12,88.6138) 
      (Apr-12,78.9129) };
   \addplot [draw=none, fill=green!30] coordinates {
      (Sep-11,75.4064)
      (Oct-11, 89.7961) 
      (Nov-11,94.4597)
      (Dec-11,76.6786) 
      (Jan-12,77.5600) 
      (Feb-12,78.2339)
      (Mar-12,88.6138) 
      (Apr-12,78.9129) };

    \legend{First Fix,Second Fix,Third Fix}
  \end{axis}
  \end{tikzpicture}

==> gfx/scatter-instance-wise.tex <==
\begin{tikzpicture}
	\begin{axis}[%
	xmin=0,
	xmax=1,
	ymin=0,
	ymax=1,
	legend pos=north west,
	extra x ticks={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
	extra y ticks={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
    tick style={grid=major},
	xlabel=HTN-BF,
	scatter/classes={%
		SMAC={mark=triangle,blue},%
		HB={mark=triangle,red},%
		BOHB={mark=triangle,magenta},
	    GGP={mark=square,brown},%
		RANDOM={mark=o,black}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.2137801696020874  0.14362035225048925  GGP
0.6007081769127165  0.5046374144871436  GGP
0.80040501293975  0.732618891275193  GGP
0.8105551882019377  0.7990912005450191  GGP
0.6130160601392632  0.253309716491257  GGP
0.6879143126177023  0.6708591606133978  GGP
0.5890306597427342  0.5157265102744979  GGP
0.5288623708542753  0.19780623735735953  GGP
0.6913172481543224  0.6930282458181473  GGP
0.5250062028242828  0.4029158635307543  GGP
0.6394154341996481  0.45812010742015097  GGP
0.6714433856970305  0.36005725977854325  GGP
0.28660500610500617  0.26547295933233434  GGP
0.5174946078434344  0.2484564590148297  GGP
0.6688158375462161  0.6279831643268682  GGP
0.7893646265560164  0.6624182803135085  GGP
0.14340381095152807  0.0  GGP
0.5724609715649456  0.382376035087634  GGP
0.3584670594129648  0.0  GGP
0.9906137063599749  0.9903174603174602  GGP
0.3756323382394412  0.2411492148844992  GGP
0.7345636433479147  0.42431593000227086  GGP
0.6842520820362815  0.3900921435529733  GGP
0.6451013144192999  0.4414339822107647  GGP
0.2137801696020874  0.1933149993081499  RANDOM
0.6007081769127165  0.0  RANDOM
0.80040501293975  0.6634911495667724  RANDOM
0.8105551882019377  0.8190420085559997  RANDOM
0.6130160601392632  0.13341961776596017  RANDOM
0.6879143126177023  0.7016764864137743  RANDOM
0.5890306597427342  0.6093463147524036  RANDOM
0.5288623708542753  0.15028453997281935  RANDOM
0.6913172481543224  0.7062768599491143  RANDOM
0.5250062028242828  0.0  RANDOM
0.6394154341996481  0.0  RANDOM
0.6714433856970305  0.03300609053162079  RANDOM
0.28660500610500617  0.2651899948342256  RANDOM
0.5174946078434344  0.265160842009287  RANDOM
0.6688158375462161  0.6641586116797696  RANDOM
0.7893646265560164  0.7934434071000459  RANDOM
0.14340381095152807  0.039997771640002136  RANDOM
0.5724609715649456  0.024875389408099684  RANDOM
0.3584670594129648  0.0  RANDOM
0.9906137063599749  0.989755120501389  RANDOM
0.3756323382394412  0.16744208146241485  RANDOM
0.7345636433479147  0.36021091542409384  RANDOM
0.6842520820362815  0.0  RANDOM
0.6451013144192999  0.044531856651629884  RANDOM
0.2137801696020874  0.15285911957144832  BOHB
0.6007081769127165  0.553051250257642  BOHB
0.80040501293975  0.7530665132453936  BOHB
0.8105551882019377  0.7663466506960089  BOHB
0.6130160601392632  0.43437499124714923  BOHB
0.6879143126177023  0.661804950228679  BOHB
0.5890306597427342  0.5892902434396243  BOHB
0.5288623708542753  0.3579679828807013  BOHB
0.6913172481543224  0.6862648824773439  BOHB
0.5250062028242828  0.4653662336689675  BOHB
0.6394154341996481  0.5206376627913896  BOHB
0.6714433856970305  0.48590838158026617  BOHB
0.28660500610500617  0.27249413220326685  BOHB
0.5174946078434344  0.3390427275478867  BOHB
0.6688158375462161  0.659999057378908  BOHB
0.7893646265560164  0.7391313393268785  BOHB
0.14340381095152807  0.11126693087179829  BOHB
0.5724609715649456  0.36253499683813195  BOHB
0.3584670594129648  0.37895028286187166  BOHB
0.9906137063599749  0.9891602593095129  BOHB
0.3756323382394412  0.39039987301387474  BOHB
0.7345636433479147  0.6076453511535125  BOHB
0.6842520820362815  0.417553320620795  BOHB
0.6451013144192999  0.45854114331994983  BOHB
0.2137801696020874  0.14627213645478487  SMAC
0.6007081769127165  0.4944807337916994  SMAC
0.80040501293975  0.740039398213987  SMAC
0.8105551882019377  0.8066309999699438  SMAC
0.6130160601392632  0.39484694723612207  SMAC
0.6879143126177023  0.6781261770244821  SMAC
0.5890306597427342  0.571696649660014  SMAC
0.5288623708542753  0.29725667427989394  SMAC
0.6913172481543224  0.698658999137755  SMAC
0.5250062028242828  0.4029158635307543  SMAC
0.6394154341996481  0.47340571785828545  SMAC
0.6714433856970305  0.45616139435724656  SMAC
0.28660500610500617  0.27120173229548233  SMAC
0.5174946078434344  0.2736222212090722  SMAC
0.6688158375462161  0.6570802591147198  SMAC
0.7893646265560164  0.7501207929921619  SMAC
0.14340381095152807  0.08224416742327394  SMAC
0.5724609715649456  0.3472285487565741  SMAC
0.3584670594129648  0.36923234656602677  SMAC
0.9906137063599749  0.9922436420808198  SMAC
0.3756323382394412  0.36966843709021774  SMAC
0.7345636433479147  0.5609819039151643  SMAC
0.6842520820362815  0.40103387637744803  SMAC
0.6451013144192999  0.4586775983298826  SMAC
0.2137801696020874  0.16982024824490577  HB
0.6007081769127165  0.5611886400490989  HB
0.80040501293975  0.7734795292165615  HB
0.8105551882019377  0.7939771372466512  HB
0.6130160601392632  0.3341529300369509  HB
0.6879143126177023  0.6777371536185094  HB
0.5890306597427342  0.5899007994754976  HB
0.5288623708542753  0.39104582053491405  HB
0.6913172481543224  0.7030605834020777  HB
0.5250062028242828  0.45874657610394853  HB
0.6394154341996481  0.5255383184382454  HB
0.6714433856970305  0.41166781726116386  HB
0.28660500610500617  0.2727162108724609  HB
0.5174946078434344  0.3598473224966246  HB
0.6688158375462161  0.6470764998759153  HB
0.7893646265560164  0.7446349700322727  HB
0.14340381095152807  0.1665282547869085  HB
0.5724609715649456  0.36230709288622676  HB
0.3584670594129648  0.35494671887557283  HB
0.9906137063599749  0.99030324567638  HB
0.3756323382394412  0.3832375960631904  HB
0.7345636433479147  0.581873281176772  HB
0.6842520820362815  0.5135939117636591  HB
0.6451013144192999  0.5023953880208023  HB
%
};
	\addlegendentry{SMAC}
	\addlegendentry{HB}
	\addlegendentry{BOHB}
	\addlegendentry{GGP}
	\addlegendentry{Random}
	\addplot[color=black] coordinates {
		(0,0)
		(1,1)
	};
	\end{axis}
\end{tikzpicture}

==> gfx/scatter-label-wise.tex <==
\begin{tikzpicture}
	\begin{axis}[%
	xmin=0,
	xmax=1,
	ymin=0,
	ymax=1,
	legend pos=north west,
	extra x ticks={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
	extra y ticks={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
    tick style={grid=major},
	xlabel=HTN-BF,
	scatter/classes={%
		SMAC={mark=triangle,blue},%
		HB={mark=triangle,red},
		BOHB={mark=triangle,magenta},
	    GGP={mark=square,brown},%
		RANDOM={mark=o,black}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.07146901799789687  0.0662375169338639  GGP
0.4023003159384584  0.22817447698764512  GGP
0.26860574688510935  0.13390481442966  GGP
0.33975876860841503  0.3323397078577976  GGP
0.41750155569773695  0.23619414458219518  GGP
0.6957848416964876  0.6844069135190884  GGP
0.2111273610532895  0.19562594485427018  GGP
0.21432900684504935  0.10166847137439743  GGP
0.5280272445407804  0.5460625808105625  GGP
0.30361857553051935  0.024546406236856187  GGP
0.22732534389186262  0.1104271287805442  GGP
0.39851506994456415  0.2680270651362429  GGP
0.4273586918019955  0.4066691361885268  GGP
0.2972064252020774  0.14554891465329475  GGP
0.47845699103561945  0.4592106315533613  GGP
0.793107345476664  0.7333266247779415  GGP
0.03681428161107929  0.0  GGP
0.2703701960524505  0.16525013935275548  GGP
0.1332128166807812  0.0  GGP
0.6361879307249677  0.6303142620466395  GGP
0.2724065697574668  0.13403805020773657  GGP
0.30986801813351994  0.16829492471863067  GGP
0.21072377527697023  0.013748908486887593  GGP
0.31869334304147057  0.04437234908443981  GGP
0.07146901799789687  0.056621593957855376  RANDOM
0.4023003159384584  0.0  RANDOM
0.26860574688510935  0.062009909049262846  RANDOM
0.33975876860841503  0.33960740217033347  RANDOM
0.41750155569773695  0.023783055658640605  RANDOM
0.6957848416964876  0.6926363789982816  RANDOM
0.2111273610532895  0.20995372908922932  RANDOM
0.21432900684504935  0.013612548290035586  RANDOM
0.5280272445407804  0.529594539971949  RANDOM
0.30361857553051935  0.0  RANDOM
0.22732534389186262  0.0  RANDOM
0.39851506994456415  0.006479896229706144  RANDOM
0.4273586918019955  0.41746427857443014  RANDOM
0.2972064252020774  0.05096988718867758  RANDOM
0.47845699103561945  0.47306507944331855  RANDOM
0.793107345476664  0.7930820045585515  RANDOM
0.03681428161107929  9.220606024275019E-4  RANDOM
0.2703701960524505  0.002580776808330988  RANDOM
0.1332128166807812  0.0  RANDOM
0.6361879307249677  0.6353957462290796  RANDOM
0.2724065697574668  0.045349417295873024  RANDOM
0.30986801813351994  0.03064660172957411  RANDOM
0.21072377527697023  0.0  RANDOM
0.31869334304147057  0.0021059653135124833  RANDOM
0.07146901799789687  0.06172381875249748  BOHB
0.4023003159384584  0.17078958710135667  BOHB
0.26860574688510935  0.21499821375138634  BOHB
0.33975876860841503  0.3325767501581299  BOHB
0.41750155569773695  0.2740637576679869  BOHB
0.6957848416964876  0.6853529818597068  BOHB
0.2111273610532895  0.20399621474802432  BOHB
0.21432900684504935  0.15814811406647628  BOHB
0.5280272445407804  0.5132907241119674  BOHB
0.30361857553051935  0.18735328284969213  BOHB
0.22732534389186262  0.14826263469108114  BOHB
0.39851506994456415  0.2811136799766602  BOHB
0.4273586918019955  0.42348357291269495  BOHB
0.2972064252020774  0.21573517233001502  BOHB
0.47845699103561945  0.47124735502001835  BOHB
0.793107345476664  0.7638875979426547  BOHB
0.03681428161107929  0.0028935428418217423  BOHB
0.2703701960524505  0.1882173770153458  BOHB
0.1332128166807812  0.10407223120588949  BOHB
0.6361879307249677  0.6386056227722895  BOHB
0.2724065697574668  0.28986822441818505  BOHB
0.30986801813351994  0.22966668826102685  BOHB
0.21072377527697023  0.15452468591959012  BOHB
0.31869334304147057  0.21999810162068476  BOHB
0.07146901799789687  0.04982614912185602  SMAC
0.4023003159384584  0.09976349667339506  SMAC
0.26860574688510935  0.16941074188557248  SMAC
0.33975876860841503  0.32310717026502944  SMAC
0.41750155569773695  0.21815728227388007  SMAC
0.6957848416964876  0.6842662178865795  SMAC
0.2111273610532895  0.1820541627840258  SMAC
0.21432900684504935  0.13869759055238035  SMAC
0.5280272445407804  0.5277281738653106  SMAC
0.30361857553051935  0.06456876643090878  SMAC
0.22732534389186262  0.16340591849930455  SMAC
0.39851506994456415  0.21570612272052045  SMAC
0.4273586918019955  0.39724984287854903  SMAC
0.2972064252020774  0.18589865748963458  SMAC
0.47845699103561945  0.4746224453451099  SMAC
0.793107345476664  0.7558550089125087  SMAC
0.03681428161107929  0.008503795655373942  SMAC
0.2703701960524505  0.14608264194014514  SMAC
0.1332128166807812  0.05444688590348281  SMAC
0.6361879307249677  0.6310035624581622  SMAC
0.2724065697574668  0.18419469669808852  SMAC
0.30986801813351994  0.2370463861521135  SMAC
0.21072377527697023  0.07688571697868771  SMAC
0.31869334304147057  0.15851322665405956  SMAC
0.07146901799789687  0.058914459405171225  HB
0.4023003159384584  0.17338686793575564  HB
0.26860574688510935  0.21203755136853863  HB
0.33975876860841503  0.32834301690753176  HB
0.41750155569773695  0.35044349948061376  HB
0.6957848416964876  0.6704871229194458  HB
0.2111273610532895  0.19628007385346188  HB
0.21432900684504935  0.15472992614521056  HB
0.5280272445407804  0.5105931930878891  HB
0.30361857553051935  0.17764471062703885  HB
0.22732534389186262  0.1662647776277107  HB
0.39851506994456415  0.3172981111664393  HB
0.4273586918019955  0.40034033044450973  HB
0.2972064252020774  0.24089365417632186  HB
0.47845699103561945  0.46881341111535935  HB
0.793107345476664  0.7574417669886297  HB
0.03681428161107929  0.03869028257104136  HB
0.2703701960524505  0.23706707088342455  HB
0.1332128166807812  0.07939729082270325  HB
0.6361879307249677  0.6347722270870418  HB
0.2724065697574668  0.32189685407064045  HB
0.30986801813351994  0.25888339330175103  HB
0.21072377527697023  0.16802478679736363  HB
0.31869334304147057  0.16982741079236005  HB
%
};
	\addlegendentry{SMAC}
	\addlegendentry{HB}
	\addlegendentry{BOHB}
	\addlegendentry{GGP}
	\addlegendentry{Random}
	\addplot[color=black] coordinates {
		(0,0)
		(1,1)
	};
	\end{axis}
\end{tikzpicture}

==> gfx/scatter-micro.tex <==
\begin{tikzpicture}
	\begin{axis}[%
	xmin=0,
	xmax=1,
	ymin=0,
	ymax=1,
	legend pos=north west,
	extra x ticks={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
	extra y ticks={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
    tick style={grid=major},
	xlabel=HTN-BF,
	scatter/classes={%
		SMAC={mark=triangle,blue},%
		HB={mark=triangle,red},
		BOHB={mark=triangle,magenta},
	    GGP={mark=square,brown},%
		RANDOM={mark=o,black}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.2440851876650123  0.26517213584218274  GGP
0.6380977172243899  0.5285690536040709  GGP
0.7617793740618027  0.6009928310204063  GGP
0.8243631825084068  0.8093024444703758  GGP
0.5914307914488816  0.3035769875635053  GGP
0.7060545841802057  0.6999707421150864  GGP
0.6069951180545049  0.564992490363024  GGP
0.5200923820783467  0.2802361525205021  GGP
0.7220833382255025  0.7067598321967974  GGP
0.5088531797656057  0.37125015793049887  GGP
0.6294998758250104  0.4333904197141198  GGP
0.6592620372610385  0.4093196347071865  GGP
0.5993329247278594  0.5447686486930651  GGP
0.494231847556662  0.2638914795598475  GGP
0.6741447235735666  0.6472271420181093  GGP
0.7827540964631392  0.732909982009318  GGP
0.1382201210590663  0.0  GGP
0.525496608159158  0.3054445807833291  GGP
0.37746177317007196  0.0  GGP
0.9913427519215956  0.9883854225566612  GGP
0.4215035105957809  0.27107536037833196  GGP
0.7051312521718682  0.4354307358234221  GGP
0.6207020768364576  0.33200871883362415  GGP
0.5890360217840604  0.4198803108177073  GGP
0.2440851876650123  0.19848104716197854  RANDOM
0.6380977172243899  0.0  RANDOM
0.7617793740618027  0.6059177088651251  RANDOM
0.8243631825084068  0.8284813659485424  RANDOM
0.5914307914488816  0.12465096554657987  RANDOM
0.7060545841802057  0.7051403353906291  RANDOM
0.6069951180545049  0.6128510683307253  RANDOM
0.5200923820783467  0.13790933108718467  RANDOM
0.7220833382255025  0.7169023410082543  RANDOM
0.5088531797656057  0.0  RANDOM
0.6294998758250104  0.0  RANDOM
0.6592620372610385  0.030054821025475652  RANDOM
0.5993329247278594  0.6025885359939718  RANDOM
0.494231847556662  0.2358287723970017  RANDOM
0.6741447235735666  0.6758719811543485  RANDOM
0.7827540964631392  0.7866239646717691  RANDOM
0.1382201210590663  0.027522522266427457  RANDOM
0.525496608159158  0.02222222222222222  RANDOM
0.37746177317007196  0.0  RANDOM
0.9913427519215956  0.989655233422671  RANDOM
0.4215035105957809  0.2002624200682102  RANDOM
0.7051312521718682  0.33798952402007315  RANDOM
0.6207020768364576  0.0  RANDOM
0.5890360217840604  0.04244558258642766  RANDOM
0.2440851876650123  0.22585648955191373  BOHB
0.6380977172243899  0.5842322432263997  BOHB
0.7617793740618027  0.717916246742676  BOHB
0.8243631825084068  0.8130978082912874  BOHB
0.5914307914488816  0.36292232022988674  BOHB
0.7060545841802057  0.6994875475675806  BOHB
0.6069951180545049  0.5982091061940455  BOHB
0.5200923820783467  0.36100631196972666  BOHB
0.7220833382255025  0.707642334614982  BOHB
0.5088531797656057  0.3842094280524256  BOHB
0.6294998758250104  0.5250701525416666  BOHB
0.6592620372610385  0.43529491318960567  BOHB
0.5993329247278594  0.5367511657554837  BOHB
0.494231847556662  0.36634156777172694  BOHB
0.6741447235735666  0.6687674023624871  BOHB
0.7827540964631392  0.7523139469978501  BOHB
0.1382201210590663  0.1137566916432059  BOHB
0.525496608159158  0.3181045040074733  BOHB
0.37746177317007196  0.3596224025334985  BOHB
0.9913427519215956  0.9906132004888777  BOHB
0.4215035105957809  0.4188571486193842  BOHB
0.7051312521718682  0.5662949886304492  BOHB
0.6207020768364576  0.48534121077025816  BOHB
0.5890360217840604  0.47838497725913404  BOHB
0.2440851876650123  0.18890166234902836  SMAC
0.6380977172243899  0.5029930365838212  SMAC
0.7617793740618027  0.6823599878425929  SMAC
0.8243631825084068  0.8178220218523526  SMAC
0.5914307914488816  0.34421425964235963  SMAC
0.7060545841802057  0.7057509544509994  SMAC
0.6069951180545049  0.585693915334931  SMAC
0.5200923820783467  0.3573763011642691  SMAC
0.7220833382255025  0.6948168064966442  SMAC
0.5088531797656057  0.37282097120640467  SMAC
0.6294998758250104  0.4778659846199715  SMAC
0.6592620372610385  0.41695039677438483  SMAC
0.5993329247278594  0.5534171601186729  SMAC
0.494231847556662  0.3188482031682966  SMAC
0.6741447235735666  0.6612367846420691  SMAC
0.7827540964631392  0.75347720516667  SMAC
0.1382201210590663  0.05625482683626011  SMAC
0.525496608159158  0.2653944084847526  SMAC
0.37746177317007196  0.32356798104787365  SMAC
0.9913427519215956  0.9924294597687702  SMAC
0.4215035105957809  0.39186929392590253  SMAC
0.7051312521718682  0.5106547872500289  SMAC
0.6207020768364576  0.3841309682149947  SMAC
0.5890360217840604  0.4679045093224305  SMAC
0.2440851876650123  0.2166310982372444  HB
0.6380977172243899  0.5737809968959569  HB
0.7617793740618027  0.7245802040002134  HB
0.8243631825084068  0.8112725228519622  HB
0.5914307914488816  0.3793546615897274  HB
0.7060545841802057  0.693311933612915  HB
0.6069951180545049  0.5945061625947363  HB
0.5200923820783467  0.3643689449514353  HB
0.7220833382255025  0.7210157981000727  HB
0.5088531797656057  0.451680962607492  HB
0.6294998758250104  0.5120728275470992  HB
0.6592620372610385  0.43694097519978203  HB
0.5993329247278594  0.5414477119497146  HB
0.494231847556662  0.39339601078383024  HB
0.6741447235735666  0.6722271344591515  HB
0.7827540964631392  0.7514287520334813  HB
0.1382201210590663  0.0927040440095074  HB
0.525496608159158  0.35491208025219  HB
0.37746177317007196  0.3555860686034245  HB
0.9913427519215956  0.9893786325876432  HB
0.4215035105957809  0.4329012808192526  HB
0.7051312521718682  0.6121037479116122  HB
0.6207020768364576  0.4529123787792516  HB
0.5890360217840604  0.5077570021732946  HB
%
};
	\addlegendentry{SMAC}
	\addlegendentry{HB}
	\addlegendentry{BOHB}
	\addlegendentry{GGP}
	\addlegendentry{Random}
	\addplot[color=black] coordinates {
		(0,0)
		(1,1)
	};
	\end{axis}
\end{tikzpicture}

==> tables/datasets.tex <==
\begin{tabular}{llllll}
\toprule
Dataset&\#I&\#L&L2IR&ULC&card.\\
\midrule
arts1 & 7484 & 26 & 0.0035 & 0.08 & 1.65\\
bibtex & 7395 & 159 & 0.0215 & 0.39 & 2.40\\
birds & 645 & 19 & 0.0295 & 0.21 & 1.01\\
bookmarks & 87856 & 208 & 0.0024 & 0.21 & 2.03\\
business1 & 11214 & 30 & 0.0027 & 0.02 & 1.60\\
computers1 & 12444 & 33 & 0.0027 & 0.03 & 1.51\\
education1 & 12030 & 33 & 0.0027 & 0.04 & 1.46\\
emotions & 593 & 6 & 0.0101 & 0.05 & 1.87\\
enron-f & 1702 & 53 & 0.0311 & 0.44 & 3.38\\
entertainment1 & 12730 & 21 & 0.0016 & 0.03 & 1.41\\
flags & 194 & 12 & 0.0619 & 0.53 & 4.12\\
genbase & 662 & 27 & 0.0408 & 0.05 & 1.25\\
health1 & 9205 & 32 & 0.0035 & 0.04 & 1.64\\
llog-f & 1460 & 75 & 0.0514 & 0.21 & 1.18\\
mediamill & 43907 & 101 & 0.0023 & 0.15 & 4.38\\
medical & 978 & 45 & 0.0460 & 0.10 & 1.25\\
recreation1 & 12828 & 22 & 0.0017 & 0.04 & 1.43\\
reference1 & 8027 & 33 & 0.0041 & 0.03 & 1.17\\
scene & 2407 & 6 & 0.0025 & 0.01 & 1.07\\
science1 & 6428 & 40 & 0.0062 & 0.07 & 1.45\\
social1 & 12111 & 39 & 0.0032 & 0.03 & 1.28\\
society1 & 14512 & 27 & 0.0019 & 0.07 & 1.67\\
tmc2007 & 28596 & 22 & 0.0008 & 0.05 & 2.16\\
yeast & 2417 & 14 & 0.0058 & 0.08 & 4.24\\
\bottomrule
\end{tabular}

==> tables/instance-wise.tex <==
\begin{tabular}{lllllll}
\toprule
Dataset&SMAC&HB&BOHB&GGP&HTN-BF&Random\\
\midrule
arts1 & .27$\pm$.05 & .36$\pm$.10 & .34$\pm$.09 & .25$\pm$.01 & \textbf{.52$\pm$.03} & .27$\pm$.09\\
bibtex & \underline{.37$\pm$.07} & \underline{.38$\pm$.06} & \textbf{.39$\pm$.03} & .24$\pm$.02 & \underline{.38$\pm$.02} & .17$\pm$.06\\
birds & \underline{.27$\pm$.04} & \underline{.27$\pm$.04} & \underline{.27$\pm$.04} & \underline{.27$\pm$.04} & \textbf{.29$\pm$.04} & \underline{.27$\pm$.04}\\
bookmarks & \underline{.08$\pm$.05} & \textbf{.17$\pm$.08} & \underline{.11$\pm$.08} & .00$\pm$.00 & \underline{.14$\pm$.03} & .04$\pm$.06\\
business1 & .74$\pm$.02 & .77$\pm$.02 & .75$\pm$.01 & .73$\pm$.01 & \textbf{.80$\pm$.02} & .67$\pm$.22\\
computers1 & .46$\pm$.05 & .50$\pm$.06 & .46$\pm$.02 & .44$\pm$.01 & \textbf{.65$\pm$.02} & .04$\pm$.13\\
education1 & .30$\pm$.07 & .39$\pm$.11 & .36$\pm$.10 & .20$\pm$.10 & \textbf{.53$\pm$.01} & .15$\pm$.15\\
emotions & .68$\pm$.05 & .68$\pm$.04 & .66$\pm$.05 & .67$\pm$.03 & \underline{.69$\pm$.04} & \textbf{.70$\pm$.04}\\
enron-f & .57$\pm$.03 & .59$\pm$.03 & .59$\pm$.03 & .52$\pm$.03 & .59$\pm$.02 & \textbf{.61$\pm$.01}\\
entertainment1 & .46$\pm$.11 & .43$\pm$.10 & .49$\pm$.14 & .36$\pm$.09 & \textbf{.67$\pm$.02} & .03$\pm$.10\\
flags & \underline{.70$\pm$.03} & \underline{.70$\pm$.04} & \underline{.69$\pm$.04} & \underline{.69$\pm$.03} & \underline{.69$\pm$.02} & \textbf{.71$\pm$.03}\\
genbase & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01}\\
health1 & .56$\pm$.10 & .58$\pm$.07 & .61$\pm$.09 & .42$\pm$.01 & \textbf{.73$\pm$.02} & .36$\pm$.18\\
llog-f & .15$\pm$.03 & .17$\pm$.04 & .15$\pm$.02 & .14$\pm$.03 & \textbf{.21$\pm$.04} & \underline{.19$\pm$.07}\\
mediamill & .50$\pm$.02 & .56$\pm$.03 & .56$\pm$.05 & .50$\pm$.00 & \textbf{.60$\pm$.03} & .00$\pm$.00\\
medical & \underline{.81$\pm$.05} & .79$\pm$.05 & \underline{.77$\pm$.09} & .80$\pm$.04 & \underline{.81$\pm$.05} & \textbf{.82$\pm$.05}\\
recreation1 & .40$\pm$.15 & .34$\pm$.11 & .42$\pm$.14 & .25$\pm$.09 & \textbf{.61$\pm$.05} & .13$\pm$.11\\
reference1 & .48$\pm$.07 & .53$\pm$.04 & .52$\pm$.04 & .46$\pm$.06 & \textbf{.64$\pm$.02} & .00$\pm$.00\\
scene & .75$\pm$.02 & .75$\pm$.03 & .74$\pm$.02 & .66$\pm$.02 & \underline{.79$\pm$.03} & \textbf{.79$\pm$.02}\\
science1 & .35$\pm$.13 & .36$\pm$.08 & .36$\pm$.12 & .38$\pm$.20 & \textbf{.57$\pm$.02} & .03$\pm$.08\\
social1 & .40$\pm$.02 & .51$\pm$.09 & .42$\pm$.14 & .39$\pm$.02 & \textbf{.68$\pm$.02} & .00$\pm$.00\\
society1 & .40$\pm$.01 & .46$\pm$.04 & .47$\pm$.04 & .40$\pm$.01 & \textbf{.52$\pm$.05} & .00$\pm$.00\\
tmc2007 & \underline{.37$\pm$.03} & \underline{.36$\pm$.02} & \textbf{.38$\pm$.02} & .00$\pm$.00 & \underline{.36$\pm$.02} & .00$\pm$.00\\
yeast & .66$\pm$.01 & .65$\pm$.02 & .66$\pm$.02 & .63$\pm$.02 & \textbf{.67$\pm$.02} & \underline{.67$\pm$.01}\\
\midrule
avg. rank & 3.71 & 2.92 & 3.33 & 4.92 & 1.67 & 4.46\\
\bottomrule
\end{tabular}

==> tables/label-wise.tex <==
\begin{tabular}{lllllll}
\toprule
& \multicolumn{6}{c}{Label-wise F-Measure} \\
&SMAC&HB&BOHB&GGP&HTN-BF&Random\\
\midrule
arts1 & .18$\pm$.09 & .24$\pm$.05 & .22$\pm$.05 & .14$\pm$.01 & \textbf{.30$\pm$.01} & .05$\pm$.08\\
bibtex & .18$\pm$.08 & \textbf{.32$\pm$.03} & \underline{.29$\pm$.06} & .14$\pm$.01 & .27$\pm$.03 & .05$\pm$.02\\
birds & \underline{.40$\pm$.05} & \underline{.40$\pm$.06} & \underline{.42$\pm$.06} & \underline{.41$\pm$.06} & \textbf{.43$\pm$.07} & \underline{.42$\pm$.06}\\
bookmarks & \underline{.01$\pm$.02} & \textbf{.04$\pm$.06} & \underline{.00$\pm$.01} & \underline{.00$\pm$.00} & \underline{.04$\pm$.04} & \underline{.00$\pm$.00}\\
business1 & .17$\pm$.06 & \underline{.22$\pm$.07} & \underline{.22$\pm$.08} & .13$\pm$.01 & \textbf{.27$\pm$.06} & .06$\pm$.06\\
computers1 & .16$\pm$.08 & .17$\pm$.05 & .22$\pm$.07 & .04$\pm$.07 & \textbf{.32$\pm$.02} & .00$\pm$.01\\
education1 & \underline{.14$\pm$.08} & .15$\pm$.05 & \underline{.16$\pm$.08} & .10$\pm$.04 & \textbf{.22$\pm$.01} & .02$\pm$.02\\
emotions & \underline{.68$\pm$.03} & \underline{.67$\pm$.04} & \underline{.68$\pm$.03} & \underline{.68$\pm$.04} & \textbf{.70$\pm$.04} & \underline{.69$\pm$.04}\\
enron-f & .18$\pm$.03 & .20$\pm$.03 & \underline{.20$\pm$.02} & \underline{.20$\pm$.02} & \textbf{.21$\pm$.03} & \underline{.21$\pm$.03}\\
entertainment1 & .22$\pm$.15 & .32$\pm$.08 & \underline{.29$\pm$.13} & .27$\pm$.09 & \textbf{.40$\pm$.03} & .01$\pm$.02\\
flags & \underline{.53$\pm$.07} & .51$\pm$.05 & \underline{.51$\pm$.06} & \textbf{.55$\pm$.07} & \underline{.53$\pm$.09} & \underline{.53$\pm$.08}\\
genbase & \underline{.63$\pm$.06} & \underline{.64$\pm$.06} & \textbf{.64$\pm$.06} & \underline{.63$\pm$.06} & \underline{.64$\pm$.07} & \underline{.64$\pm$.06}\\
health1 & \underline{.24$\pm$.11} & \underline{.26$\pm$.07} & .23$\pm$.11 & .17$\pm$.02 & \textbf{.31$\pm$.02} & .03$\pm$.02\\
llog-f & .05$\pm$.01 & .06$\pm$.02 & \underline{.06$\pm$.02} & \underline{.07$\pm$.01} & \textbf{.07$\pm$.01} & \underline{.06$\pm$.02}\\
mediamill & .10$\pm$.05 & .17$\pm$.05 & .17$\pm$.06 & .23$\pm$.01 & \textbf{.40$\pm$.05} & .00$\pm$.00\\
medical & \underline{.32$\pm$.03} & \underline{.33$\pm$.04} & \underline{.33$\pm$.03} & \underline{.33$\pm$.03} & \textbf{.34$\pm$.04} & \textbf{.34$\pm$.03}\\
recreation1 & .22$\pm$.16 & \underline{.35$\pm$.08} & \underline{.29$\pm$.13} & .24$\pm$.06 & \textbf{.42$\pm$.14} & .02$\pm$.02\\
reference1 & \underline{.17$\pm$.07} & \underline{.17$\pm$.05} & .15$\pm$.08 & .11$\pm$.03 & \textbf{.23$\pm$.06} & .00$\pm$.00\\
scene & .76$\pm$.02 & .76$\pm$.02 & .76$\pm$.02 & .73$\pm$.03 & \underline{.79$\pm$.02} & \textbf{.79$\pm$.02}\\
science1 & .15$\pm$.11 & \underline{.24$\pm$.05} & .20$\pm$.07 & .17$\pm$.07 & \textbf{.27$\pm$.03} & .00$\pm$.01\\
social1 & .08$\pm$.06 & \underline{.17$\pm$.08} & \underline{.16$\pm$.09} & .02$\pm$.01 & \textbf{.21$\pm$.02} & .00$\pm$.00\\
society1 & .06$\pm$.08 & .18$\pm$.06 & .19$\pm$.08 & .02$\pm$.00 & \textbf{.30$\pm$.02} & .00$\pm$.00\\
tmc2007 & \underline{.05$\pm$.08} & \underline{.08$\pm$.10} & \underline{.10$\pm$.11} & .00$\pm$.00 & \textbf{.13$\pm$.11} & .00$\pm$.00\\
yeast & \underline{.47$\pm$.01} & \underline{.47$\pm$.01} & \underline{.47$\pm$.01} & .46$\pm$.01 & \textbf{.48$\pm$.01} & \underline{.47$\pm$.01}\\
\midrule
avg. rank & 4.46 & 3.25 & 2.92 & 4.42 & 1.33 & 4.63\\
\bottomrule
\end{tabular}

==> tables/micro.tex <==
\begin{tabular}{lllllll}
\toprule
Dataset&SMAC&HB&BOHB&GGP&HTN-BF&Random\\
\midrule
arts1 & .32$\pm$.12 & .39$\pm$.05 & .37$\pm$.08 & .27$\pm$.01 & \textbf{.50$\pm$.01} & .24$\pm$.08\\
bibtex & \underline{.39$\pm$.07} & \textbf{.43$\pm$.02} & \underline{.42$\pm$.04} & .27$\pm$.02 & \underline{.42$\pm$.02} & .20$\pm$.09\\
birds & .55$\pm$.04 & .54$\pm$.06 & .54$\pm$.04 & \underline{.55$\pm$.05} & \underline{.60$\pm$.05} & \textbf{.60$\pm$.06}\\
bookmarks & .06$\pm$.02 & \underline{.09$\pm$.06} & \underline{.11$\pm$.06} & .00$\pm$.00 & \textbf{.14$\pm$.05} & .03$\pm$.04\\
business1 & .68$\pm$.03 & .72$\pm$.03 & .72$\pm$.04 & .60$\pm$.20 & \textbf{.76$\pm$.02} & .60$\pm$.20\\
computers1 & .47$\pm$.08 & .51$\pm$.06 & .48$\pm$.06 & .42$\pm$.01 & \textbf{.59$\pm$.04} & .04$\pm$.13\\
education1 & .36$\pm$.11 & .37$\pm$.10 & .36$\pm$.11 & .30$\pm$.06 & \textbf{.52$\pm$.01} & .14$\pm$.14\\
emotions & \underline{.71$\pm$.04} & \underline{.69$\pm$.04} & \underline{.70$\pm$.05} & \underline{.70$\pm$.03} & \textbf{.71$\pm$.03} & \underline{.70$\pm$.04}\\
enron-f & .59$\pm$.02 & .60$\pm$.02 & .60$\pm$.02 & .57$\pm$.02 & \underline{.61$\pm$.02} & \textbf{.61$\pm$.01}\\
entertainment1 & .42$\pm$.11 & .45$\pm$.10 & .43$\pm$.09 & .41$\pm$.09 & \textbf{.66$\pm$.01} & .03$\pm$.09\\
flags & .70$\pm$.03 & \underline{.72$\pm$.03} & \underline{.71$\pm$.03} & \underline{.71$\pm$.03} & \textbf{.72$\pm$.03} & \underline{.72$\pm$.03}\\
genbase & \textbf{.99$\pm$.01} & \underline{.99$\pm$.01} & \textbf{.99$\pm$.01} & \underline{.99$\pm$.01} & \underline{.99$\pm$.01} & \underline{.99$\pm$.01}\\
health1 & .51$\pm$.12 & .61$\pm$.04 & .57$\pm$.07 & .44$\pm$.02 & \textbf{.71$\pm$.03} & .34$\pm$.17\\
llog-f & .19$\pm$.05 & .22$\pm$.04 & .22$\pm$.03 & \textbf{.26$\pm$.04} & \underline{.25$\pm$.05} & .20$\pm$.08\\
mediamill & .50$\pm$.02 & .57$\pm$.06 & .58$\pm$.04 & .53$\pm$.00 & \textbf{.64$\pm$.02} & .00$\pm$.00\\
medical & \underline{.82$\pm$.04} & \underline{.81$\pm$.04} & \underline{.81$\pm$.04} & .81$\pm$.04 & \underline{.82$\pm$.04} & \textbf{.83$\pm$.04}\\
recreation1 & .34$\pm$.16 & .38$\pm$.11 & .36$\pm$.14 & .30$\pm$.02 & \textbf{.59$\pm$.04} & .12$\pm$.10\\
reference1 & .48$\pm$.06 & .51$\pm$.05 & .53$\pm$.06 & .43$\pm$.02 & \textbf{.63$\pm$.02} & .00$\pm$.00\\
scene & .75$\pm$.02 & .75$\pm$.02 & .75$\pm$.02 & .73$\pm$.03 & \underline{.78$\pm$.02} & \textbf{.79$\pm$.02}\\
science1 & .27$\pm$.10 & .35$\pm$.12 & .32$\pm$.13 & .31$\pm$.13 & \textbf{.52$\pm$.03} & .02$\pm$.07\\
social1 & .39$\pm$.02 & .45$\pm$.10 & .49$\pm$.10 & .33$\pm$.12 & \textbf{.62$\pm$.08} & .00$\pm$.00\\
society1 & .37$\pm$.01 & .45$\pm$.04 & .39$\pm$.14 & .37$\pm$.01 & \textbf{.51$\pm$.02} & .00$\pm$.00\\
tmc2007 & .32$\pm$.07 & \underline{.36$\pm$.06} & \underline{.36$\pm$.06} & .00$\pm$.00 & \textbf{.38$\pm$.02} & .00$\pm$.00\\
yeast & .66$\pm$.02 & \underline{.67$\pm$.02} & \underline{.67$\pm$.01} & .65$\pm$.01 & \textbf{.68$\pm$.02} & \underline{.68$\pm$.01}\\
\midrule
avg. rank & 4.00 & 3.04 & 3.13 & 4.96 & 1.33 & 4.54\\
\bottomrule
\end{tabular}

==> tables/vertically-merged.tex <==
\begin{tabular}{llrrrrrr}
\toprule
&Dataset&SMAC&HB&BOHB&GGP&HTN-BF&Random\\
\midrule
\multirow{25}{*}{\rotatebox{90}{Instance-Wise F-Measure ($F_I$)}}
&arts1 & .27$\pm$.05 & .36$\pm$.10 & .34$\pm$.09 & .25$\pm$.01 & \textbf{.52$\pm$.03} & .27$\pm$.09\\
&bibtex & \underline{.37$\pm$.07} & \underline{.38$\pm$.06} & \textbf{.39$\pm$.03} & .24$\pm$.02 & \underline{.38$\pm$.02} & .17$\pm$.06\\
&birds & \underline{.27$\pm$.04} & \underline{.27$\pm$.04} & \underline{.27$\pm$.04} & \underline{.27$\pm$.04} & \textbf{.29$\pm$.04} & \underline{.27$\pm$.04}\\
&bookmarks & \underline{.08$\pm$.05} & \textbf{.17$\pm$.08} & \underline{.11$\pm$.08} & .00$\pm$.00 & \underline{.14$\pm$.03} & .04$\pm$.06\\
&business1 & .74$\pm$.02 & .77$\pm$.02 & .75$\pm$.01 & .73$\pm$.01 & \textbf{.80$\pm$.02} & .67$\pm$.22\\
&computers1 & .46$\pm$.05 & .50$\pm$.06 & .46$\pm$.02 & .44$\pm$.01 & \textbf{.65$\pm$.02} & .04$\pm$.13\\
&education1 & .30$\pm$.07 & .39$\pm$.11 & .36$\pm$.10 & .20$\pm$.10 & \textbf{.53$\pm$.01} & .15$\pm$.15\\
&emotions & .68$\pm$.05 & .68$\pm$.04 & .66$\pm$.05 & .67$\pm$.03 & \underline{.69$\pm$.04} & \textbf{.70$\pm$.04}\\
&enron-f & .57$\pm$.03 & .59$\pm$.03 & .59$\pm$.03 & .52$\pm$.03 & .59$\pm$.02 & \textbf{.61$\pm$.01}\\
&entertainment1 & .46$\pm$.11 & .43$\pm$.10 & .49$\pm$.14 & .36$\pm$.09 & \textbf{.67$\pm$.02} & .03$\pm$.10\\
&flags & \underline{.70$\pm$.03} & \underline{.70$\pm$.04} & \underline{.69$\pm$.04} & \underline{.69$\pm$.03} & \underline{.69$\pm$.02} & \textbf{.71$\pm$.03}\\
&genbase & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01}\\
&health1 & .56$\pm$.10 & .58$\pm$.07 & .61$\pm$.09 & .42$\pm$.01 & \textbf{.73$\pm$.02} & .36$\pm$.18\\
&llog-f & .15$\pm$.03 & .17$\pm$.04 & .15$\pm$.02 & .14$\pm$.03 & \textbf{.21$\pm$.04} & \underline{.19$\pm$.07}\\
&mediamill & .50$\pm$.02 & .56$\pm$.03 & .56$\pm$.05 & .50$\pm$.00 & \textbf{.60$\pm$.03} & .00$\pm$.00\\
&medical & \underline{.81$\pm$.05} & .79$\pm$.05 & \underline{.77$\pm$.09} & .80$\pm$.04 & \underline{.81$\pm$.05} & \textbf{.82$\pm$.05}\\
&recreation1 & .40$\pm$.15 & .34$\pm$.11 & .42$\pm$.14 & .25$\pm$.09 & \textbf{.61$\pm$.05} & .13$\pm$.11\\
&reference1 & .48$\pm$.07 & .53$\pm$.04 & .52$\pm$.04 & .46$\pm$.06 & \textbf{.64$\pm$.02} & .00$\pm$.00\\
&science1 & .35$\pm$.13 & .36$\pm$.08 & .36$\pm$.12 & .38$\pm$.20 & \textbf{.57$\pm$.02} & .03$\pm$.08\\
&social1 & .40$\pm$.02 & .51$\pm$.09 & .42$\pm$.14 & .39$\pm$.02 & \textbf{.68$\pm$.02} & .00$\pm$.00\\
&society1 & .40$\pm$.01 & .46$\pm$.04 & .47$\pm$.04 & .40$\pm$.01 & \textbf{.52$\pm$.05} & .00$\pm$.00\\
&tmc2007 & \underline{.37$\pm$.03} & \underline{.36$\pm$.02} & \textbf{.38$\pm$.02} & .00$\pm$.00 & \underline{.36$\pm$.02} & .00$\pm$.00\\
&yeast & .66$\pm$.01 & .65$\pm$.02 & .66$\pm$.02 & .63$\pm$.02 & \textbf{.67$\pm$.02} & \textbf{.67$\pm$.01}\\
\cmidrule{2-8}
& avg. rank & 3.71 & 2.92 & 3.33 & 4.92 & 1.67 & 4.46\\
%\toprule
%Dataset&SMAC&HB&BOHB&GGP&HTN-BF&Random\\
\midrule
\multirow{25}{*}{\rotatebox{90}{Label-Wise F-Measure ($F_L$)}}
&arts1 & .18$\pm$.09 & .24$\pm$.05 & .22$\pm$.05 & .14$\pm$.01 & \textbf{.30$\pm$.01} & .05$\pm$.08\\
&bibtex & .18$\pm$.08 & \textbf{.32$\pm$.03} & \underline{.29$\pm$.06} & .14$\pm$.01 & .27$\pm$.03 & .05$\pm$.02\\
&birds & \underline{.40$\pm$.05} & \underline{.40$\pm$.06} & \underline{.42$\pm$.06} & \underline{.41$\pm$.06} & \textbf{.43$\pm$.07} & \underline{.42$\pm$.06}\\
&bookmarks & \underline{.01$\pm$.02} & \textbf{.04$\pm$.06} & \underline{.00$\pm$.01} & \underline{.00$\pm$.00} & \textbf{.04$\pm$.04} & \underline{.00$\pm$.00}\\
&business1 & .17$\pm$.06 & \underline{.22$\pm$.07} & \underline{.22$\pm$.08} & .13$\pm$.01 & \textbf{.27$\pm$.06} & .06$\pm$.06\\
&computers1 & .16$\pm$.08 & .17$\pm$.05 & .22$\pm$.07 & .04$\pm$.07 & \textbf{.32$\pm$.02} & .00$\pm$.01\\
&education1 & \underline{.14$\pm$.08} & .15$\pm$.05 & \underline{.16$\pm$.08} & .10$\pm$.04 & \textbf{.22$\pm$.01} & .02$\pm$.02\\
&emotions & \underline{.68$\pm$.03} & \underline{.67$\pm$.04} & \underline{.68$\pm$.03} & \underline{.68$\pm$.04} & \textbf{.70$\pm$.04} & \underline{.69$\pm$.04}\\
&enron-f & .18$\pm$.03 & .20$\pm$.03 & \underline{.20$\pm$.02} & \underline{.20$\pm$.02} & \textbf{.21$\pm$.03} & \textbf{.21$\pm$.03}\\
&entertainment1 & .22$\pm$.15 & .32$\pm$.08 & \underline{.29$\pm$.13} & .27$\pm$.09 & \textbf{.40$\pm$.03} & .01$\pm$.02\\
&flags & \underline{.53$\pm$.07} & .51$\pm$.05 & \underline{.51$\pm$.06} & \textbf{.55$\pm$.07} & \underline{.53$\pm$.09} & \underline{.53$\pm$.08}\\
&genbase & \underline{.63$\pm$.06} & \textbf{.64$\pm$.06} & \textbf{.64$\pm$.06} & \underline{.63$\pm$.06} & \textbf{.64$\pm$.07} & \textbf{.64$\pm$.06}\\
&health1 & \underline{.24$\pm$.11} & \underline{.26$\pm$.07} & .23$\pm$.11 & .17$\pm$.02 & \textbf{.31$\pm$.02} & .03$\pm$.02\\
&llog-f & .05$\pm$.01 & .06$\pm$.02 & \underline{.06$\pm$.02} & \textbf{.07$\pm$.01} & \textbf{.07$\pm$.01} & \underline{.06$\pm$.02}\\
&mediamill & .10$\pm$.05 & .17$\pm$.05 & .17$\pm$.06 & .23$\pm$.01 & \textbf{.40$\pm$.05} & .00$\pm$.00\\
&medical & \underline{.32$\pm$.03} & \underline{.33$\pm$.04} & \underline{.33$\pm$.03} & \underline{.33$\pm$.03} & \textbf{.34$\pm$.04} & \textbf{.34$\pm$.03}\\
&recreation1 & .22$\pm$.16 & \underline{.35$\pm$.08} & \underline{.29$\pm$.13} & .24$\pm$.06 & \textbf{.42$\pm$.14} & .02$\pm$.02\\
&reference1 & \underline{.17$\pm$.07} & \underline{.17$\pm$.05} & .15$\pm$.08 & .11$\pm$.03 & \textbf{.23$\pm$.06} & .00$\pm$.00\\
&scene & .76$\pm$.02 & .76$\pm$.02 & .76$\pm$.02 & .73$\pm$.03 & \textbf{.79$\pm$.02} & \textbf{.79$\pm$.02}\\
&science1 & .15$\pm$.11 & \underline{.24$\pm$.05} & .20$\pm$.07 & .17$\pm$.07 & \textbf{.27$\pm$.03} & .00$\pm$.01\\
&social1 & .08$\pm$.06 & \underline{.17$\pm$.08} & \underline{.16$\pm$.09} & .02$\pm$.01 & \textbf{.21$\pm$.02} & .00$\pm$.00\\
&society1 & .06$\pm$.08 & .18$\pm$.06 & .19$\pm$.08 & .02$\pm$.00 & \textbf{.30$\pm$.02} & .00$\pm$.00\\
&tmc2007 & \underline{.05$\pm$.08} & \underline{.08$\pm$.10} & \underline{.10$\pm$.11} & .00$\pm$.00 & \textbf{.13$\pm$.11} & .00$\pm$.00\\
&yeast & \underline{.47$\pm$.01} & \underline{.47$\pm$.01} & \underline{.47$\pm$.01} & .46$\pm$.01 & \textbf{.48$\pm$.01} & \underline{.47$\pm$.01}\\
\cmidrule{2-8}
&avg. rank & 4.46 & 3.25 & 2.92 & 4.42 & 1.33 & 4.63\\
%\toprule
%Dataset&SMAC&HB&BOHB&GGP&HTN-BF&Random\\
\midrule
\multirow{25}{*}{\rotatebox{90}{Micro-Averaged F-Measure ($F_\mu$)}}
&arts1 & .32$\pm$.12 & .39$\pm$.05 & .37$\pm$.08 & .27$\pm$.01 & \textbf{.50$\pm$.01} & .24$\pm$.08\\
&bibtex & \underline{.39$\pm$.07} & \textbf{.43$\pm$.02} & \underline{.42$\pm$.04} & .27$\pm$.02 & \underline{.42$\pm$.02} & .20$\pm$.09\\
&birds & .55$\pm$.04 & .54$\pm$.06 & .54$\pm$.04 & \underline{.55$\pm$.05} & \textbf{.60$\pm$.05} & \textbf{.60$\pm$.06}\\
&bookmarks & .06$\pm$.02 & \underline{.09$\pm$.06} & \underline{.11$\pm$.06} & .00$\pm$.00 & \textbf{.14$\pm$.05} & .03$\pm$.04\\
&business1 & .68$\pm$.03 & .72$\pm$.03 & .72$\pm$.04 & .60$\pm$.20 & \textbf{.76$\pm$.02} & .60$\pm$.20\\
&computers1 & .47$\pm$.08 & .51$\pm$.06 & .48$\pm$.06 & .42$\pm$.01 & \textbf{.59$\pm$.04} & .04$\pm$.13\\
&education1 & .36$\pm$.11 & .37$\pm$.10 & .36$\pm$.11 & .30$\pm$.06 & \textbf{.52$\pm$.01} & .14$\pm$.14\\
&emotions & \textbf{.71$\pm$.04} & \underline{.69$\pm$.04} & \underline{.70$\pm$.05} & \underline{.70$\pm$.03} & \textbf{.71$\pm$.03} & \underline{.70$\pm$.04}\\
&enron-f & .59$\pm$.02 & .60$\pm$.02 & .60$\pm$.02 & .57$\pm$.02 & \textbf{.61$\pm$.02} & \textbf{.61$\pm$.01}\\
&entertainment1 & .42$\pm$.11 & .45$\pm$.10 & .43$\pm$.09 & .41$\pm$.09 & \textbf{.66$\pm$.01} & .03$\pm$.09\\
&flags & .70$\pm$.03 & \underline{.72$\pm$.03} & \underline{.71$\pm$.03} & \underline{.71$\pm$.03} & \textbf{.72$\pm$.03} & \textbf{.72$\pm$.03}\\
&genbase & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01} & \textbf{.99$\pm$.01}\\
&health1 & .51$\pm$.12 & .61$\pm$.04 & .57$\pm$.07 & .44$\pm$.02 & \textbf{.71$\pm$.03} & .34$\pm$.17\\
&llog-f & .19$\pm$.05 & .22$\pm$.04 & .22$\pm$.03 & \textbf{.26$\pm$.04} & \underline{.25$\pm$.05} & .20$\pm$.08\\
&mediamill & .50$\pm$.02 & .57$\pm$.06 & .58$\pm$.04 & .53$\pm$.00 & \textbf{.64$\pm$.02} & .00$\pm$.00\\
&medical & \underline{.82$\pm$.04} & \underline{.81$\pm$.04} & \underline{.81$\pm$.04} & .81$\pm$.04 & \underline{.82$\pm$.04} & \textbf{.83$\pm$.04}\\
&recreation1 & .34$\pm$.16 & .38$\pm$.11 & .36$\pm$.14 & .30$\pm$.02 & \textbf{.59$\pm$.04} & .12$\pm$.10\\
&reference1 & .48$\pm$.06 & .51$\pm$.05 & .53$\pm$.06 & .43$\pm$.02 & \textbf{.63$\pm$.02} & .00$\pm$.00\\
&scene & .75$\pm$.02 & .75$\pm$.02 & .75$\pm$.02 & .73$\pm$.03 & \underline{.78$\pm$.02} & \textbf{.79$\pm$.02}\\
&science1 & .27$\pm$.10 & .35$\pm$.12 & .32$\pm$.13 & .31$\pm$.13 & \textbf{.52$\pm$.03} & .02$\pm$.07\\
&social1 & .39$\pm$.02 & .45$\pm$.10 & .49$\pm$.10 & .33$\pm$.12 & \textbf{.62$\pm$.08} & .00$\pm$.00\\
&society1 & .37$\pm$.01 & .45$\pm$.04 & .39$\pm$.14 & .37$\pm$.01 & \textbf{.51$\pm$.02} & .00$\pm$.00\\
&tmc2007 & .32$\pm$.07 & \underline{.36$\pm$.06} & \underline{.36$\pm$.06} & .00$\pm$.00 & \textbf{.38$\pm$.02} & .00$\pm$.00\\
&yeast & .66$\pm$.02 & \underline{.67$\pm$.02} & \underline{.67$\pm$.01} & .65$\pm$.01 & \textbf{.68$\pm$.02} & \textbf{.68$\pm$.01}\\
\cmidrule{2-8}
&avg. rank & 4.00 & 3.04 & 3.13 & 4.96 & 1.33 & 4.54\\
\bottomrule
\end{tabular}
